A Multi-technique Study of the Dynamical Evolution of the Viscous Disk around the Be Star {\omega} CMa

There is an increasing body of evidence that suggests that Be disks are well described by the Viscous Decretion Disk (VDD) model according to which the formation and structure of the disk depend on the kinematic viscosity of the gas. However, most observational tests of the VDD to-date were done for systems that do not display strong temporal variability. From this analysis we (1) obtain a realistic physical model of the circumstellar environment; (2) measure the viscosity parameter of the gas, both during the formation and dissipation phases of the disk; (3) obtain a reliable estimate of the stellar mass and angular momentum loss rates during outburst. Our simulations suggests that the VDD model adequately describes the structural evolution of the disk. Furthermore, our analysis allowed us to determine the viscosity parameter a, as well as the net mass and angular momentum (AM) loss rates. We find that a is variable, ranging from 0.1 to 1.0, not only from cycle to cycle but also within a given cycle. Additionally, build-up phases have larger values of a than the dissipation phases. We also find that, contrary to what is generally assumed, during dissipation the outward AM flux is not necessarily zero, meaning that {\omega} CMa does not experience a true quiescence but, instead, switches between a high AM loss rate state to a low AM loss rate one during which the disk quickly assumes an overall lower density but never zero. We confront the average AM loss rate with predictions from stellar evolution models for fast-rotating stars, and find that our measurements are smaller by more than one order of magnitude. The model developed using the V-band photometry as a constraint was applied to several other observables. Overall, the results of this multi-technique study were very positive, with a good match for multi-band photometry, polarization, and most spectroscopic characteristics.

==> tex/bibliografia.tex <==
\bibitem{Quireza et al. 2007}{quireza}Quireza C., Rocha-Pinto H. J., Maciel W. J., 2007, A\&A, 475, 217

\bibitem[Aoki et al.(2001)]{2001ApJ...561..346A} Aoki, W., Ryan, S. G., Norris, J. E., Beers, T. C., Ando, H., Iwamoto, N., Kajino, T., Mathews, G. J., \& Fujimoto, M. Y. 2001, ApJ 561, 346

\bibitem[Aoki et al.(2002)]{2002ApJ...580.1149A} Aoki, W., Ryan, S. G., Norris, J. E., Beers, T. C., Ando, H., \& Tsangarides, S. 2002, ApJ 580, 1149 

\bibitem[Wasserburg et al. (1994)]{1994ApJ...424..412W} Wasserburg, G. J., Busso, M., Gallino, R., \& Raiteri, C. M. 1994, ApJ 424, 412

